Investigating Speech Features for Continuous Turn-Taking Prediction Using LSTMs

For spoken dialog systems to conduct fluid conversational interactions with users, the systems must be sensitive to turn-taking cues produced by a user. Models should be designed so that effective decisions can be made as to when it is appropriate, or not, for the system to speak. Traditional end-of-turn models, where decisions are made at utterance end-points, are limited in their ability to model fast turn-switches and overlap. A more flexible approach is to model turn-taking in a continuous manner using RNNs, where the system predicts speech probability scores for discrete frames within a future window. The continuous predictions represent generalized turn-taking behaviors observed in the training data and can be applied to make decisions that are not just limited to end-of-turn detection. In this paper, we investigate optimal speech-related feature sets for making predictions at pauses and overlaps in conversation. We find that while traditional acoustic features perform well, part-of-speech features generally perform worse than word features. We show that our current models outperform previously reported baselines.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> tables/coarse_feature_table_acoustic_groupings.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &  test\ losses &  f_1\ 50ms &  f_1\ 500ms &  f_1\ overlap\ &  f_1\ short\ long \\
\midrule
Energy                       &     0.561845 &       0.728012 &        0.759302 &                               0.638932 &             0.738296 \\
Spectral                     &     0.555577 &       0.746561 &        0.780080 &                               0.671997 &             \textbf{0.772666*} \\
Frequency                    &     0.584483 &       0.686092 &        0.742894 &                               0.645236 &             0.689693 \\
VA Energy                    &     0.556966 &       0.756522 &        0.755949 &                               0.659003 &             0.738052 \\
VA Spectral                  &     \textbf{0.548611} &       \textbf{0.778478} &        \textbf{0.787119} &                               \textbf{0.686846} &             0.766541 \\
VA Frequency                 &     0.559705 &       0.752454 &        0.760228 &                               0.640533 &             0.707916 \\
VA Energy Spectral           &     \textbf{0.546423*} &       \textbf{0.782765*} &        \textbf{0.793642*} &                               \textbf{0.683842} &             \textbf{0.770013} \\
VA Spectral Frequency        &     0.548850 &       \textbf{0.778248} &        0.786236 &                               \textbf{0.691684*} &             \textbf{0.767048} \\
VA Energy Frequency          &     0.553060 &       0.765440 &        0.773881 &                               0.682547 &             0.746183 \\
VA Energy Spectral Frequency &     \textbf{0.547047} &       0.777099 &        \textbf{0.791629} &                               0.680524 &             0.763831 \\
\bottomrule
\end{tabular}


==> tables/coarse_feature_table_with_va.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &  test\ losses &  f_1\ 50ms &  f_1\ 500ms &  f_1\ overlap\ &  f_1\ short\ long \\
\midrule
VA                 &     0.573542 &       0.690298 &        0.706431 &                               0.580650 &             0.635155 \\
VA Acous           &     0.547042 &       0.780811 &        0.794663 &                               \textbf{0.678879} &             \textbf{0.764512*} \\
VA BNFs            &     0.557239 &       0.764192 &        0.790087 &                               0.655822 &             0.729066 \\
VA POS             &     0.571818 &       0.715395 &        0.711231 &                               0.587866 &             0.640931 \\
VA Words           &     0.559805 &       0.756252 &        0.754636 &                               0.638219 &             0.703662 \\
VA Ling            &     0.557588 &       0.767302 &        0.760439 &                               0.631109 &             0.702882 \\
VA Acous BNFs      &     0.551840 &       0.778686 &        0.799157 &                               \textbf{0.681845} &             0.742625 \\
VA Acous Words     &     \textbf{0.545486*} &       \textbf{0.788631} &        \textbf{0.804938} &                               0.653653 &             0.758092 \\
VA Acous POS       &     \textbf{0.546323} &       0.782142 &        0.796371 &                               \textbf{0.693089*} &             \textbf{0.763591} \\
VA Acous Ling      &     \textbf{0.546454} &       \textbf{0.793631*} &        0.802136 &                               0.658335 &             \textbf{0.759042} \\
VA BNFs Ling       &     0.551259 &       0.783805 &        \textbf{0.809661} &                               0.655187 &             0.736696 \\
VA Acous BNFs Ling &     0.546673 &       \textbf{0.790223} &        \textbf{0.813317*} &                               0.667792 &             0.756666 \\
\bottomrule
\end{tabular}


==> tables/coarse_feature_table_with_va_main_groups.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &  test\ losses &  f_1\ 50ms &  f_1\ 500ms &  f_1\ overlap\ &  f_1\ short\ long \\
\midrule
VA                 &     0.573542 &       0.690298 &        0.706431 &                               0.580650 &             0.635155 \\
VA Acous           &     \textbf{0.547042} &       0.780811 &        0.794663 &                               \textbf{0.678879} &             \textbf{0.764512*} \\
VA BNFs            &     0.557239 &       0.764192 &        0.790087 &                               0.655822 &             0.729066 \\
VA Ling            &     0.557588 &       0.767302 &        0.760439 &                               0.631109 &             0.702882 \\
VA Acous BNFs      &     0.551840 &       0.778686 &        0.799157 &                               \textbf{0.681845*} &             0.742625 \\
VA Acous Ling      &     \textbf{0.546454*} &       \textbf{0.793631*} &        \textbf{0.802136} &                               0.658335 &             \textbf{0.759042} \\
VA BNFs Ling       &     0.551259 &       \textbf{0.783805} &        \textbf{0.809661} &                               0.655187 &             0.736696 \\
VA Acous BNFs Ling &     \textbf{0.546673} &       \textbf{0.790223} &        \textbf{0.813317*} &                               \textbf{0.667792} &             \textbf{0.756666} \\
\bottomrule
\end{tabular}


==> tables/coarse_feature_table_without_va.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &  test\ losses &  f_1\ 50ms &  f_1\ 500ms &  f_1\ overlap\ &  f_1\ short\ long \\
\midrule
Acous           &     \textbf{0.550968} &       0.759677 &        0.795706 &                               \textbf{0.67656*}0 &             0.757037 \\
BNFs            &     0.569257 &       0.723283 &        0.774554 &                               0.617042 &             0.710557 \\
Pos             &     0.625807 &       0.643079 &        0.618603 &                               0.323092 &             0.568487 \\
Words           &     0.582457 &       0.707550 &        0.725268 &                               0.578636 &             0.706563 \\
Ling            &     0.580253 &       0.709521 &        0.735241 &                               0.584493 &             0.693611 \\
Acous BNFs      &     0.555128 &       \textbf{0.765719} &        0.801185 &                               0.670240 &             \textbf{0.76261}0 \\
Acous Words     &     0.550985 &       0.763649 &        0.796542 &                               \textbf{0.672485} &             0.758232 \\
Acous POS       &     0.552119 &       0.751870 &        0.785988 &                               0.659113 &             \textbf{0.76761}0 \\
Acous Ling      &     \textbf{0.549142*} &       \textbf{0.771403} &        \textbf{0.806079} &                               0.661428 &             0.758180 \\
BNFs Ling       &     0.557417 &       0.764510 &        \textbf{0.810685} &                               0.645581 &             0.743382 \\
Acous BNFs Ling &     \textbf{0.550711} &       \textbf{0.778063*} &        \textbf{0.815917*} &                               \textbf{0.673423} &             \textbf{0.768509*} \\
\bottomrule
\end{tabular}


==> tables/coarse_feature_table_without_va_main_groups.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} &  test\ losses &  f_1\ 50ms &  f_1\ 500ms &  f_1\ overlap\ &  f_1\ short\ long \\
\midrule
Acous           &     \textbf{0.550968} &       0.759677 &        0.795706 &                               \textbf{0.67656*}0 &             0.757037 \\
BNFs            &     0.569257 &       0.723283 &        0.774554 &                               0.617042 &             0.710557 \\
Ling            &     0.580253 &       0.709521 &        0.735241 &                               0.584493 &             0.693611 \\
Acous BNFs      &     0.555128 &       \textbf{0.765719} &        0.801185 &                               \textbf{0.67024}0 &             \textbf{0.76261}0 \\
Acous Ling      &     \textbf{0.549142*} &       \textbf{0.771403} &        \textbf{0.806079} &                               0.661428 &             \textbf{0.75818}0 \\
BNFs Ling       &     0.557417 &       0.764510 &        \textbf{0.810685} &                               0.645581 &             0.743382 \\
Acous BNFs Ling &     \textbf{0.550711} &       \textbf{0.778063*} &        \textbf{0.815917*} &                               \textbf{0.673423} &             \textbf{0.768509*} \\
\bottomrule
\end{tabular}

